QUOKA: Query-Oriented KV Selection For Efficient LLM Prefill

We present QUOKA: Query-oriented KV selection for efficient attention, a training-free and hardware agnostic sparse attention algorithm for accelerating transformer inference under chunked prefill. While many queries focus on a smaller group of keys in the attention operator, we observe that queries with low cosine similarity with respect to the mean query interact more strongly with more keys and have the greatest contribution to final attention logits. By prioritizing these low cosine similarity queries, the behavior of full attention during the prefill stage can be closely approximated. QUOKA leverages this observation, accelerating attention by (1) first retaining a small set of representative queries and (2) then subselectin the keys most aligned with those queries. Through experiments on Needle-In-A-Haystack, LongBench, RULER, and Math500, we show that, while realizing a 3x reduction in time-to-first-token, 5x speedup in attention on Nvidia GPUs and up to nearly a 7x speedup on Intel Xeon CPUs, QUOKA achieves near-baseline accuracy, utilizing 88% fewer key-value pairs per attention evaluation.

==> contents/_introduction.tex <==
\section{Introduction}

With the rapid advances of large language models (LLMs), long-context inference tasks such as chain-of-thought reasoning or agentic generation have become increasingly crucial. However, in such regimes, the quadratic complexity of attention mechanisms \citep{vaswani2017attention} becomes a significant bottleneck for fast inference. Additionally, in practical edge LLM systems (e.g., consumer-grade GPUs or mobile devices), the memory bandwidth cost of transferring KV-cache between memory and compute units further exacerbates the latency.

Sparse attention \needref{} addresses these challenges by exploiting inherent sparsity in attention weights (i.e., the softmax output often contains mostly near-zero values). Typical sparse attention methods reduce latency during generation by identifying a subset of KV entries that are likely to attend to a current query, thereby avoiding the full attention computation. 

Despite remarkable speed-ups during the generation phase, sparse attention methods rarely optimize the prefill phase, which accounts for a substantial portion of end-to-end latency in long-context inference. Existing approaches \needref{} that accelerate prefill often require considerable custom kernel development, \textcolor{red}{limiting portability beyond well-studied hardware such as NVIDIA GPUs.}

To address this, we propose \ourmethodfull{}, a training-free, \textcolor{red}{hardware-agnostic?}, sparse attention mechanism optimized for the prefill phase. Utilizing chunked prefill, \ourmethod{} divides the input context into blocks. Within each block, we identify active KV pairs by ranking keys based on cosine similarity to the query vectors within the block, and keep only the most relevant pairs. These selected KV pairs and block queries are then processed using an existing dense attention kernel (e.g., FlashAttention). 

By reducing the size of the KV-cache used in attention, our method significantly reduces both memory transfer and compute, which is especially beneficial on resource-constrained hardware. Furthermore, \ourmethod{} utilizes hyperparameters which allow practitioners to trade off accuracy with latency reduction and to select a configuration optimized for their specific hardware latency profile. 


We evaluate \ourmethod{} on tasks X, Y, Z, demonstrating an X× speed-up in attention computation compared to FlashAttention, Y, Z and an overall A\% reduction in end-to-end latency during prefill. Our contributions are as follows:
\begin{itemize}[leftmargin=*]
\item A
\item B
\item C
\end{itemize}
 

==> contents/background.tex <==
\section{Background}
\label{sec:background}
\subsection{Transformers and Attention}
Transformers have become the dominant sequence-modeling paradigm since \cite{vaswani2017attention}. A transformer block consists of two main computational steps: the attention operator and a feed-forward network (FFN).
In this work, we focus primarily on the computational aspects of attention.
For an input sequence $X = [x_1, \ldots, x_T]$, we define the attention operator $\mathrm{Attn}(X)$ as
\begin{equation}
\label{eq:attention}
\mathrm{Attn}(X) = \mathrm{Softmax}\left( \frac{QK^\top}{\sqrt{d}} + M \right)V = AV,
\end{equation}

where keys $K = XW_K $, queries $Q= XW_Q$ and values $V=XW_V$ are learned projections of the input tokens with $W_K, W_Q, W_v$ in $\mathbb{R}^{d \times d}$ and $M$ is a causal mask with zeros below the diagonal and $-\infty$ elsewhere.

\subsection{Sources of LLM inference latency}

%\textcolor{red}{Junyoung: We'd like to claim sparse attention with a minimal active KV cache selection overhead + chunked prefill would solve the TTFT problem. Regarding that we mainly want to accuse the prefill bottleneck is large attention matrix or KV cache transfer? I'm not sure. Feel free to educate me
%Matt: not sure i understand your point. prefill is compute bound so less attention comp is best (achieved by using fewer KVs). generation is memory bound so eventually KV cache transfer becomes a bottleneck with long enough generation lengths}

Autoregressive text generation with a transformer model is divided into a \textit{prompt prefill} stage and a \textit{text generation} stage. 
Each stage has unique algorithmic characteristics that cause different performance bottlenecks, each of which must be addressed in turn.
\paragraph{Prefill latency}
The prefill stage requires processing all tokens of the input prompt and \textit{prefilling} the KV cache with keys and values (KVs).
This entails propagating each token through the entire model to compute the KVs in each layer.
Attention must compute $T^2$ inner products of $q_ik_j^T$ between $T$ KVs and $T$ queries.
The feedforward network must then be applied to each of the $T$ attention outputs.
This means for long input sequences, attention is the bottleneck of the prefill phase.

FlashAttention \citep{dao2022flashattention,dao2023flashattention,shah2024flashattention} helps to overcome this by tuning the attention operator to leverage hardware-specific characteristics, \textcolor{red}{such as optimal tiling and work partitioning, tensor core utilization, overlapping computation and communication, and datatype-specific hardware acceleration.}
However, this does not fundamentally reduce the computational complexity of prefill: the total number of queries and KVs involved in the attention computation must be reduced in order to explicitly overcome the quadratic complexity.
To complicate matter further, in order to achieve a practical algorithmic speed-up, this reduction must be done in a manner that \textcolor{red}{(i) is compatible with FlashAttention improvements and (ii) runs in sub-quadratic time.}

\paragraph{Generation latency}
The situation is different during the token generation stage. 
The attention operator attends to a single query and $T$ KVs, so the complexity is no longer an obstacle.
For short generation lengths, the computation is memory-bound: the large feedforward network weights saturate memory bandwidth and compute units are often waiting for tensors to be loaded from slow system memory to fast shared memory. 
This is an inherent limitation of current LLMs, \needref{although steps are being taken in this direction}.  
However, as generation lengths grow longer, such as during reasoning tasks or agentic code generation, the memory footprint of the KV cache will surpass the network weights and will consume most of the memory bandwidth.
Reducing the number of KVs required in each attention evaluation will bound the memory transfer and accelerate generation-intensive tasks.



\subsection{Chunked Prefill}

Due to the causality enforced in \cref{eq:attention}, $X$ can be processed in sequential \textit{chunks} \citep{agrawal2023sarathi,holmes2024deepspeed}.
We can partition $X$ into non-overlapping chunks of size $b$:
$X = [X_0, X_1, \ldots, X_{B-1}]$, where $X_i = [x_{bi}, \ldots, x_{b(i+1)-1}]$ and $B = \lceil T/b \rceil$.
For chunk $i$, let $K_{<i}$ and $V_{<i}$ denote the concatenation of keys and values from all preceding chunks.
Then:
\begin{equation}
\label{eq:block_attention}
\mathrm{Attn}(X_i) \;=\; \mathrm{Softmax}\!\left(
\frac{Q_i [\,K_i \;|\; K_{<i}\,]^\top}{\sqrt{d}} + M_i \right)
[\,V_i \;|\; V_{<i}\,],
\end{equation}
where $[\,\cdot \;|\; \cdot\,]$ denotes concatenation along the sequence dimensions and the mask $M_i$ enforces causality within $X_i$ and against future tokens.
%This \emph{chunked prefill} is critical for inference on mobile or consumer hardware, where memory bandwidth and capacity are limited; by choosing an appropriate block size $b$, practitioners can trade computation for memory traffic to optimize end-to-end LLM inference latency.
%Processing the input prompt using \textit{chunked prefill} \citep{agrawal2023sarathi} involves processing $B$ prompt tokens at a time to compute $B$ KVs in each decoder layer before generation.
Chunked prefill is important for inference on edge devices, such as mobile devices or consumer GPUs, where memory bandwidth and quantity is limited. 
\needref{Compute graph compilers and custom hardware accelerators can squeeze out additional performance from chunked prefill due to the static tensor sizes and optimized scheduling.}
Chunked prefill also improves cloud inference latency and throughput by interleaving prefill and decode requests, which increases overall GPU utilization \citep{holmes2024deepspeed,agrawal2025efficient}.
The token generation inference phase can also be interpreted as chunked prefill with $b=1$ and a non-empty KV cache. 

%Although mathematically equivalent to full attention, chunked prefill can degrade downstream benchmark performance when integrated with acceleration techniques like KV cache eviction, attention sparsification and \needref{others}. \textcolor{red}{This is because information/scope is limited, cite keydiff paper tova etc...

% Although mathematically equivalent to full attention, chunked prefill can degrade downstream benchmark performance when integrated with attention acceleration techniques. 
% %This is because information/scope is limited, cite keydiff paper tova etc...
% This is because many prefill acceleration methods prune KVs using a token importance metric or compression scheme \citep{oren2024transformers}.
% Both approaches are challenging without access to the entire sequence, but chunked prefill can only process chunks sequentially \needref{cite something else about chunked prefill perf loss}. 

%REPHRASE and combine. 
%KV caching methods also take a performance hit under chunked prefill, but recent methods have taken steps to address this \citep{park2025keydiff}.
%While KV caching can bound the number of KVs in the attention operation, many tokens are still required to match the full baseline performance.
%\needref{also (other methods)}. PLEASE SPECIFY LIMITATIONS TO OTHER METHODS 

%\textcolor{red}{on the other hand selective attention takes a different approach but is also not tailored towards chunked prefill. Selective attention is a promising approach to speed up the prefill phase, but also suffers during chunked prefill. describe the benefits of this approach and then enumerate the limitations (only focus on TPS? not applicable to chunked prefill, etc etc, see section 4) of other methods detailed in section 4}


\subsection{Attention sparsity}
\label{subsec:attn_sparsity}
% \begin{itemize}
%     \item Methods (token eviction, sparse attn)
%     \item limitation -- they tend to focus on TPS problem more? but why? maybe they do not adopt chunked prefill during prefill? do we want to tell the readers they would fail by referencing our experiment tables?
% \end{itemize}

% The high sparsity of attention matrix $A$ is commonly found in various pre-trained LLM \citep{zhang2024h2o,xiaoefficient, oren2024transformers, zhu2024sampleattention, yang2024tidaldecode, park2025keydiff}. For instance, \cite{zhang2024h2o} reports 95\% sparsity in attention scores and that they follow a power-law distribution with few tokens contributing most of each score's magnitude. 

% During the generation phase of LLM, this inherent sparsity in $A$ is used to reduce its computational overhead in \cref{eq:attention}, by sub-selcting KVs from $K$ and $V$ having high alignment score $\alpha$ (e.g., $qK^\top$, or $\mathrm{Sotfmax}(qK^\top)$) against to the current query $q$ as follows:
% \begin{align}
% \label{eq:sparse_attention}
% \mathrm{SparseAttn}(q,K,V) &= \mathrm{Softmax}\left( \frac{q\hat{K}^\top}{\sqrt{d}} + M \right)\hat{V}, \\
% I &= \texttt{TopK}(\alpha, n), \\
% \hat{K}&=\texttt{gather}(K, I), \\ 
% \hat{V}&=\texttt{gather}(V, I)
% \end{align}

% However, those sparse attention methods often focus on generation phase where measuring the alignment of KV to a single query $q$ is essential.

% \paragraph{Chunked Prefill and Sparse Attention} Adopting sparse attention (\cref{eq:sparse_attention}) to each block in chunked prefill (\cref{eq:block_attention}) provides a natural prefill speed-up as the size of $A$ is bounded to the size of selected KV cache and thus compute the attention output in a sub-quartic way. Unlike the generation phase, the sparse attention requires to subselect KV aligned with multiple queries. As shown in \cref{table:longbench_compare}, a naive extension of sparse attention methods to this multi-query setup showing a significant down-stream task performance. This implies a dedicated routine to select KV cache (finish this) to provide a prefill speedup with a minimal performance degradation.


% involving a subset of KV cache in \cref{eq:attention} selected by the alignment score


% using either a custom attention mask $M$ or decreasing the number of KVs used in \cref{eq:attention}.


Many studies \citep{zhang2024h2o,xiaoefficient, oren2024transformers, zhu2024sampleattention, yang2024tidaldecode, park2025keydiff} have observed that attention matrices of decoder-only transformer models tend to be very sparse. For instance, \citep{zhang2024h2o} reports 95\% sparsity in attention scores and that they follow a power-law distribution with few tokens  contributing most of each score's magnitude.  
This sparsity often occurs in the form of \textit{attention sinks}, where a special token in each attention head attracts the majority of the score \citep{barbero2025llms}. 
Empirically, this prevents token over-mixing and rank collapse within heads and helps heads implement single-token retrieval patterns \citep{olsson2022context}. %Sparsity also appears to be the result of training dynamics causing entropy collapse within attention distributions \citep{anonymous2025variance}.

This inherent sparsity in the attention operator can be used to reduce its computational overhead, using either a custom attention mask $M$ or decreasing the number of KVs used in \cref{eq:attention}.
%If the attention sparsity pattern was known a priori, it would be possible to significantly reduce the computational burden of attention without impacting the performance of the LLM, either through masking or by reducing the number of KV pairs included in the computation.
%Several papers \citep{yang2024tidaldecode, zhu2024sampleattention, singhania2024loki}, efficiently approximate attention to estimate key importance, then subselect KV-pairs used in the attention computation based on these scores, significantly increasing the efficiency of the operation. MJM consolidated this below
KV cache eviction methods are one approach to sparsify the attention operator. 
A subset of KVs across the input prompt and generated tokens are stored as an approximation of the full token sequence up to a fixed cache budget. 
While KV cache eviction is an effective acceleration method for LLM inference, it does have some limitations.
A large KV cache size is needed to match the eviction-free benchmark performance, limiting potential latency improvements \citet{park2025keydiff}. \needref{finish this, add another sparse attention method, FlexPrefill, SpecPrefill, flexattention, sageattention (oops not sparse)??}

Selective attention is a promising direction to directly leverage inherent attention sparsity. 
Instead of attending over all queries and KVs for each token, selective attention applies a dynamic heuristic to determine which KVs contribute significantly to the final attention score over the current set of tokens.
\citep{leviathan2024selective} showed that a selective attention heuristic can actually improve downstream benchmark scores; subsequent work \citep{yang2024tidaldecode,zhu2024sampleattention,singhania2024loki, ribar2023sparq,lai2025flexprefill} have solidified this claim with competing approaches.

\subsubsection{Chunked Prefill and Attention Sparsity Challenges}
Despite the potential benefits of recent sparse attention methods, many challenges remain applying them in a chunked prefill setting. 
The primary concern is that many schemes cause benchmark performance degradation under chunked prefill. 
KV cache eviction methods often rely on an attention-based heuristics to determine which KVs to evict.
Attention-based eviction on a per-chunk basis can cause premature eviction. Recent methods have made attempts to address this \citep{park2025keydiff}, but many tokens must be retained to approach baseline performance and thereby limiting acceleration potential.
% selective attentions methods that attend to a single query and why they are lame
Selective attention methods also suffer in the chunked prefill setting
Attention-based selection criteria suffer when trying to simultaneously select the best keys for a entire chunk of queries. 
\citep{zhao2019explicit,tang2024quest,ribar2024sparq,tang2024quest,singhania2024loki,yang2024tidaldecode} all provide various methods for selecting important KVs for a given single query, but break down when applied to multiple queries simultaneously. 
Selective attention methods have been proposed that handle many queries \citep{zhang2025spargeattn,gao2024seerattention,zhu2024sampleattention, jiang2024minference, lai2025flexprefill}, but still have several shortcomings. 
The main challenges for multi-query selective attention methods are: (i) simple integration into an existing chunked prefill system like \citep{kwon2023efficient}; (ii) straightforward implementation without custom CUDA kernels to achieve competitive performance (simplifying FlashAttention integration and cross-platform support); (iii) seamless KV cache eviction compatibility; and (iv) minimizing downstream benchmark degradation when used during chunked prefill.

%\needref{MJM still WIP... standby}
%KV caching methods also take a performance hit under chunked prefill, but recent methods have taken steps to address this \citep{park2025keydiff}.
%While KV caching can bound the number of KVs in the attention operation, many tokens are still required to match the full baseline performance.
%\needref{also (other methods)}. PLEASE SPECIFY LIMITATIONS TO OTHER METHODS 
%\textcolor{red}{on the other hand selective attention takes a different approach but is also not tailored towards chunked prefill. Selective attention is a promising approach to speed up the prefill phase, but also suffers during chunked prefill. describe the benefits of this approach and then enumerate the limitations (only focus on TPS? not applicable to chunked prefill, etc etc, see section 4) of other methods detailed in section 4}
%Several papers \citep{yang2024tidaldecode, zhu2024sampleattention, singhania2024loki}, efficiently approximate attention to estimate key importance, then subselect KV-pairs used in the attention computation based on these scores, significantly increasing the efficiency of the operation. 
%\textcolor{red}{on the other hand selective attention takes a different approach but is also not tailored towards chunked prefill. Selective attention is a promising approach to speed up the prefill phase, but also suffers during chunked prefill. describe the benefits of this approach and then enumerate the limitations (only focus on TPS? not applicable to chunked prefill, etc etc, see section 4) of other methods detailed in section 4}

%However, many of these approaches have two major drawbacks: difficult integration with FlashAttention and poor downstream performance when applying chunked prefill during inference.
\textcolor{red}{
\begin{itemize}
    \item previous methods are myopic
    \item Geometric properties of Q and K subselection via max
    \item GQA pre-aggregation and reduction via mean
    \item softmax approximation via cosine similarity (attention scores are unbounded
\end{itemize}
\ourmethod{} stages
\begin{itemize}
    \item QueryDiff: subselect $N_Q$ queries from the current chunk (because not all queries contribute significantly to attention (something related to Dalton's figure from ppt)) [Goal: reduce number of queries involved in attention map]
    \item average significant queries (i.e. output of QueryDiff) over the KV groups. This reduces computation by $n_Q/n_{KV}$
    \item Cosine similarity between important queries and all keys,    
    \item Reduce cos-sim along num queries dimension to produce a score for each key. We use max to avoid missing outlying score (rather than means which can accidentally skip important keys for a given query)??? Looking for "worst case" score
\end{itemize}
Main difference from competitors
\begin{itemize}
    \item we subselect keys and queries using geometry
    \item reduce queries over KV heads before cossim by linearity of mean(cossim(...)) to speed up scoring
    \item max aggregation over queries to retain outlying keys 
\end{itemize}
}
% KV caching/Block -> Sparse attention as a solution for LLM latency solution?


% maybe we can mention KV caching here with one sentence? coz it is so well adopted; we don't really need to explain it a lot? 


%With these factors in mind, we propose \ourmethod{}

% to this end, we propose \ourmethod...

% \begin{itemize}
%     \item BPP is great!
%     \item BPP makes life hard
%     \item KV caching is hard with BPP, need a lot of tokens to match baseline perf
%     \item something is hard with BPP bc we said so
%     \item something else is hard with BPP bc we said so
%     \item Selective attention is great
% \end{itemize}

% (decoding a single toke with KV cache is a special)


==> contents/introduction.tex <==
\section{Introduction}
With the rapid advances of large language models (LLMs), deployment is no longer confined to high-end datacenter GPUs: there is growing demand for efficient inference on heterogeneous hardware, including consumer-grade GPUs, CPUs, and even edge devices such as laptops and mobile devices. In such settings, long-context inference tasks such as chain-of-thought reasoning and agentic generation are increasingly crucial, but the quadratic complexity of attention mechanism \citep{vaswani2017attention} becomes a significant bottleneck for fast inference. For example, processing a prompt of length 32k tokens on a 7B LLM can consume up to 60--70\% of the end-to-end latency, even before the first output token is generated. This overhead is particularly severe in real-world deployments, where users submit long prompts but expect interactive response times.

Sparse attention \citep{ribar2023sparq, zhao2019explicit} is a promising approach to mitigate this cost by exploiting the empirical sparsity of attention distributions, where most scores are near zero. Such methods have been successfully applied to the \textit{generation} stage, where each new query attends only to the most relevant cached keys and values (KVs). Some recent research attempts to accelerate the \textit{prefill} stage as well, but they typically do so via kernel-level modifications tightly coupled to specific hardware. While effective on those platforms, such approaches require substantial engineering effort and hinder portability to CPUs, mobile devices, and emerging accelerators. Because inference today must run across a wide spectrum of hardware, a kernel-level path is difficult to generalize. By contrast, we take a structural view: combining chunked prefill with chunk-wise KV subselection via efficient attention estimation to enable prefill speedups without custom kernels.

Chunked prefill \citep{agrawal2023sarathi,agrawal2025efficient} partitions the input sequence into chunks, allowing each to be processed sequentially with improved locality and compatibility with efficient dense kernels such as FlashAttention \citep{dao2022flashattention,dao2023flashattention,shah2024flashattention}. Within this formulation, applying sparse attention chunk-wise is a natural way to reduce prefill cost. However, reusing methods designed for the generation phase —where sparsity is guided by a single query—does leads to severe accuracy degredation in the multi-query setting of prefill. Moreover, utilizing sparse attention methods designed for prefill without chunking leads to similar loss of performance. These gaps highlight the need for dedicated KV selection strategies tailored for chunked prefill.

To address this challenge, we propose \ourmethodfull{}, a \textbf{training-free and hardware-agnostic sparse attention mechanism} optimized for prefill. By exploiting the geometry of queries and keys, in particular, that attention to each key is dominated by a small subset of queries identifiable by their angular similarity, \ourmethod{} reduces the KV cache while preserving accuracy and efficiency. Unlike prior approaches that rely on custom kernels, our method requires only standard operations—cosine similarity, normalization, and top-$k$ selection—which are universally supported across CPUs, GPUs, and edge accelerators. The reduced KV sets produced by our method can be passed directly to hardware-optimized kernels (e.g., FlashAttention) without modification. In other words, our speedup arises from reducing the effective problem size rather than exploiting hardware-specific features, ensuring both efficiency and portability.

\ourmethod{} introduces three design choices motivated by geometric insights into query–key interactions: (1) \textit{query subselection} to reduce redundancy by retaining only the most informative queries; (2) \textit{group-aware aggregation} to ensure compatibility with grouped-query attention (GQA); and (3) \textit{cosine-similarity scoring} to provide a stable, bounded proxy for softmax-based importance. By reducing the effective KV set during prefill, our approach achieves sub-quadratic complexity while maintaining high accuracy. This yields substantial latency reductions on both consumer-grade GPUs and edge hardware, where memory bandwidth is often the primary bottleneck. We demonstrate that \ourmethod{} achieves an 5$\times$ speed-up in attention computation and an overall $3\times$ reduction in end-to-end prefill latency, with negligible accuracy loss across benchmarks.

Our contributions are threefold:
\begin{itemize}[leftmargin=*]
\item We provide the first sparse attention method specifically optimized for LLM inference using chunked prefill.
\item We introduce \ourmethod{}, a geometry-guided, training-free, hardware-agnostic algorithm that integrates seamlessly with dense attention kernels without requiring custom primitives.
\item We provide theoretical justification and empirical validation, showing that our method reduces end to end prefill latency by up to $3\times$ while preserving task performance across long-context benchmarks.
\end{itemize}


% 



==> contents/method.tex <==
\section{Method}
As discussed in \cref{subsec:attn_sparsity}, estimates of attention scores can be used to determine token importance and subselect KV pairs most relevant to attention. Competing approaches feature a scoring function $f(Q,K)$ that
\begin{enumerate}
    \item \emph{Subselects} $Q$ as $\hat{Q}$ along the sequence or channel dimension for more efficient score computation;
    \item \emph{Computes a score} $S \approx \hat{Q}K^\top$ reflecting attention sparsity;
    \item \emph{Aggregates} $S$ along both query dimension and among key value groups in GQA to obtain a single score for each key for subselection;
\end{enumerate}
Our work develops an algorithm compatible with chunked prefill that \emph{subselects queries $Q$}, \emph{computes scores $S$} and \emph{aggregates scores} to subselect KVs $\hat{K}, \hat{V}$ to approximately solve \cref{eq:min_attention}. 
The competing approaches in \cref{subsec:attn_sparsity}  utilize the mean for score aggregation which doesn't robustly handle outlying scores. This interacts poorly with their use of un-normalized attention logits to compute $S$, which exacerbates information loss from aggregation. Finally, the geometric properties of keys and queries within attention explored in \citep{park2025keydiff} suggest a way to subselect $Q$ without degrading our measurement of token importance. We describe our specific design choices within this framework below.

\subsection{Subselecting Queries}
\cite{park2025keydiff} has shown that, in decoder-only transformers, keys and queries have a distinctive geometric structure. While \cite{park2025keydiff} study key geometry, we focus on the geometry of queries. 
Given a fixed key token, the sparsity of attention heads guarantees that most attention weights corresponding to this token will be dominated by a small number of queries. We show this with the sample attention output in \cref{fig:attention}, where the queries between index $30-40$ have consistently high activation. By only utilizing consistently important queries to score for KV subselection, we reduce the computational complexity for scoring without losing significant information for key token importance.
This means that the method we use to subselect queries should keep queries that contribute most to attention scores. 

We show that these query tokens can be readily identified through their angular distance with the average query. This is formalized in the following result:
%Given a fixed key token, the sparsity of attention heads guarantees that most attention weights corresponding to this token will be dominated by a small number of queries. We show this with the sample attention output in \cref{fig:attention}, where the queries between index $30-40$ have consistently high activation. By only utilizing consistently important queries to score for KV subselection, we reduce the computational complexity for scoring without losing significant information for key token importance. We show that these query tokens can be readily identified through their angular distance with the average query. This is formalized in the following result:
\begin{theorem}\label{theorem:keydiff-key-query}
Consider a fixed query $q_0$ and key $k$ and let the average of a set of queries be denoted $M_Q$. Suppose $\textrm{CosSim}({k}, q_0) = \beta_q > 0$ and $\textrm{CosSim}(M_Q, k) = \alpha_q < 0$. Then 
\begin{equation}
\textrm{CosSim}(M_Q, {q^*}) \leq 1 + \alpha_q \beta_q - 0.5\alpha_q^2 -0.5\beta_q^2.
\label{eq:key-query-eq}
\end{equation}
\end{theorem}

Proof of this result follows directly from Theorem \textcolor{red}{$3.2$} in \citep{park2025keydiff}. 

We can conclude from \cref{theorem:keydiff-key-query} that if a $q^*$ attends strongly to $k$, $\beta_q$ will be large and $\alpha_q$ will be small. This means that the metric we use to select the queries, $S_Q = -\textrm{CosSim}(M_Q, {q^*})$ will be large when $q^*$ is very unaligned with $M_Q$ and align more with $k$. 
\par\medskip
\begin{wrapfigure}{c}{.45\linewidth}
    \includegraphics[width=0.95\linewidth]{figures/attention_plot.pdf}
    \caption{The attention matrix taken from layer $1$ of the Llama3.2-3B-Instruct model. The attention pattern is sparse, with weight predominantly allocated on a subset of queries and keys.}
    \label{fig:attention}
    \vspace{-2mm}
\end{wrapfigure}

\subsection{Scoring via Cosine Similarity}
\label{subsec:scoring}
Given the reduced set of queries, the next step is to evaluate their interactions with keys. Existing
methods often use raw dot products $QK^{\top}$, but these are scale-dependent and unstable under aggregation.
Instead, \ourmethod{} computes
\[
S = \mathrm{CosSim}(Q, K),
\]
which normalizes vectors to unit length and provides a bounded, geometry-aware proxy for softmax
attention weights. Recent work \citep{mongaras2025cottention,park2025keydiff} also supports the use of cosine similarity as a lightweight normalization that approximates softmax behavior. Empirically, ablations on the RULER benchmark \citep{hsieh2024ruler} show that cosine similarity improves subselection quality by about 10\% compared to the dot product, as reported in \textcolor{red}{Table X} and \textcolor{red}{Figure X}. 

% \subsection{Computing Score for Subselection}
% % \input{tables/ablation_cossim}

% While most algorithms compute $S$ as $QK^\top$ recent work \citep{mongaras2025cottention,park2025keydiff} suggests that the cosine similarity between queries and keys better captures semantic relationships between tokens. They demonstrate that cosine similarity normalizes attention weights similarly to the softmax operation without the high computational burden. 
% We make use of this fact here and define our pre-aggregated score as $S = \textrm{CosSim}(Q, K)$. The results of an ablation study using the RULER benchmark \citep{hsieh2024ruler} validate this choice by demonstrating a $10\%$ increase in performance using cosine similarity over the dot product. % We hypothesize this occurs since angular relationships predict the importance of relationships between keys and queries better than the dot product as in \citep{park2025keydiff} and because cosine similarity acts an inexpensive form of score normalization, allowing all queries to operate on the same scale in a similar way to the softmax operator.


\subsection{Aggregation Across Queries and KV Groups}
\label{subsec:score_aggregation}
After scoring, aggregation is required along two axes: across queries and across grouped-query attention (GQA) heads.

For the query axis, averaging scores can obscure rare but important query--key interactions: if only a few queries strongly attend to a key, their contribution is diluted by the majority of weak queries. To prevent this, \ourmethod{} uses the \textbf{maximum} across queries, which robustly preserves such outliers. As shown in \textcolor{red}{Table X}, this choice yields substantially better performance than mean aggregation on the RULER benchmark.

For the GQA axis, we introduce a \textit{pre-aggregation} method that averages scores across KV groups \emph{before} computing attention. Unlike the query axis, head-level token importance is known to be highly correlated \citep{bhojanapalli2021leveraging}, making the \textbf{mean} aggregation both accurate and stable. Crucially, pre-aggregation reduces the effective computation and memory bandwidth by a factor proportional to the number of KV groups, and is a key component enabling compatibility with modern architectures.


\subsection{Chunked Prefill with \ourmethod{}}
The three components described above—query subselection, scoring, and aggregation—are integrated
into the overall \emph{chunked prefill} process. For each incoming block $X_i$ in the input sequence, \ourmethod{}
reduces the active KV set using the procedure in \cref{alg:ourmethod}. The resulting subset of keys and values is then passed to the attention computation for that chunk. 

% This process is summarized in Algorithm~\ref{alg:geoselect_chunked_prefill}.

% \begin{algorithm}[t]
% \caption{Chunked Prefill with \ourmethod{}}
% \label{alg:geoselect_chunked_prefill}
% \begin{algorithmic}[1]
% \Require Input sequence $X = [X_0, X_1, \ldots, X_{B-1}]$, chunk size $L$, KV budget $B_{\text{SA}}$
% \State Initialize output list $\mathcal{Y} \gets [\;]$
% \For{each chunk $X_i$}
%     \State Compute queries $Q_i$, keys $K_i$, values $V_i$
%     \State Concatenate cache: $K_{\leq i} = [K_{<i} \mid K_i], \; V_{\leq i} = [V_{<i} \mid V_i]$
%     \State $(\hat{K}, \hat{V}) \gets \textsc{Geoselect}(Q_i, K_{\leq i}, V_{\leq i}, B_{\text{SA}})$
%     \State $Y_i \gets \textsc{Attention}(Q_i, \hat{K}, \hat{V})$
%     \State Append $Y_i$ to $\mathcal{Y}$
%     \State $K_{<i+1} \gets K_{\leq i}, \; V_{<i+1} \gets V_{\leq i}$
% \EndFor
% \State \Return $Y \gets \mathrm{Concat}(\mathcal{Y})$
% \end{algorithmic}
% \end{algorithm}

By reducing the KV budget at each chunk, \ourmethod{} shrinks both compute and memory transfer
costs. This enables significant prefill acceleration while maintaining accuracy across long-context
benchmarks.




% \subsection{Aggregation}
% \paragraph{Aggregation across queries}


% Aggregation from $S = \textrm{CosSim}(Q, K)$ must occur across two axes: the query sequence dimension and the key value groups. In the latter case, we found that a simple mean appears to best combine the scoring information across query heads. The reason for this is the relative uniformity of token scores across heads \citep{bhojanapalli2021leveraging}. In the former, however, our studies determined that using the max to aggregate scores resulted in significantly less selective attention performance loss. This is due to the wide variation in score magnitude for keys across queries which can be seen in \cref{fig:attention} and in results such as \citep{mylonas2024attention}. If the mean is utilized to aggregate over queries keys which have high attention logits with a small number of queries, and may be very important in prefill will receive a small score and may not be included in the KV subselection. Hence, using the maximum for aggregation is a better choice to robustly capture the effect of outliers. As further evidence of this, \cref{table:ruler_ablation} shows the results of the RULER benchmark using both mean and max across the query dimension. %As seen in \cref{fig:attention}, often only a single pair of $Q, K$ tokens result in a high attention score. In order to ensure such keys are retained, we utilize the max.




% \paragraph{GQA and pre-aggregation across KV groups}

% GQA \citep{ainslie2023gqa} is a ubiquitous variant of multi-head attention \citep{vaswani2017attention}, where multiple heads share the same KV pairs. This increases inference efficiency by shrinking the KV-cache size and lowering memory bandwidth costs. In our case, computing key token importance using attention scores with GQA requires aggregation over key-value groups. Modern models such as Llama3, Qwen3, Gemma, and GPT-OSS \citep{yang2025qwen3, team2025gemma, dubey2024llama, agarwal2025gpt}  typically use $3-8\times$ more query heads than KV heads and hence consideration of this feature in sparse attention methods is important for compatibility with modern and future architectures. Additionally, leveraging this compression is critical to the efficiency of our method.

% GQA complicates computing key token importance using attention scores since attention scores are computed across all query heads. Hence, we need to properly aggregate these scores across key-value groups to disambiguate the scores for each key. 
\input{tables/ablation_mean}

%Our experiments demonstrated that taking the mean of the scores across these groups yields the best results.

%since token importance is correlated across heads, it makes sense to take the average?
% Research on MHA shows that token importance is highly correlated across heads \citep{bhojanapalli2021leveraging}. In this case, it makes sense to aggregate scores across heads using a mean, since those scores are likely to be similar and have few outliers. Note that due to the linearity of the mean and $QK^\top$, we can average the queries across the key-value groups first before computing $QK^\top$, reducing the complexity of the computation by a factor commensurate with the number of key-value groups. This significantly reduces both the computational complexity and memory bandwidth requirements of the attention score estimation which can be used to determine key importance.

% In our case, we will compute a proxy of the softmax attention using the cosine similarity between keys and queries. To apply the same GQA aggregation trick, we simply need to normalize the queries before computing their mean across the key-value groups.







% \subsection{Motivation}


% \paragraph{Softmax regularization and approximation}
% \cite{saratchandran2024rethinking} suggests that the efficacy of softmax in attention isn't simply due to its probabilistic normalization, but rather because it implicitly regularizes the Frobenius norm of the attention map during training. This can prevent weights from exploding, improving generalization. 

% One of the major difficulties encountered by algorithms such as SampleAttention \citep{zhu2024sampleattention} is that trying to use attention logits to estimate token importance can lead to erroneous results. This is due to the fact that if more than one query token is present in the computation, each row of the attention matrix $QK^\top$ may have significantly different scaling that would otherwise be smoothed by the regularization effects of the softmax. Hence, in order to get an accurate estimate of key token importance, we need to either compute the softmax, which is expensive due to the exponential, max-scanning, casting and summing required, or use another technique. As noted in \cref{subsec:attn_sparsity}, many algorithms, \sout{including \ourmethod{}}, seek to efficiently estimate these scores to reduce the KV-pairs utilized in the attention computation.  

% \paragraph{Geometric properties of keys and queries} \cite{park2025keydiff} shows that the cosine similarity between keys and queries is remarkably correlated. Experiments demonstrate that attention weights, when aggregated over key value groups and queries, have high Spearman rank correlation coefficient with aggregated cosine similarities. This indicates that the cosine similarity between keys and queries can regularize attention scores in a similar way to the softmax by bounding scores between $q_i and k_j$ at a fraction of the computational cost. We ran an ablation over the RULER benchmark, varying only the scoring method, either using attention logits or the cosine similarity between keys and queries in \cref{table:ruler_ablation_cossim} where it was apparent that the cosine similarity appears to better recall important tokens into the attention computation. Because cosine similarity can be defined as the dot product of two $\ell_2$ normalized vectors, during chunked prefill we may cache the key norms to avoid recomputation and increase efficiency. We also note that using the cosine similarity between queries and keys may increase the scores of important keys. For example, it's well known \citep{barbero2025llms} that the sink key often has small norm but has high cosine similarity with most queries. In this case, using the cosine similarity increases the score of such a token, and leads the algorithm to prioritize the retention of information regardless of key norm.



% \cite{park2025keydiff, barbero2025llms} demonstrate that in order for attention heads to have a high degree of both selectivity and sparsity, the keys and queries must have very particular geometric properties. In particular, they show that most keys and queries have negative cosine similarity. This suppresses their attention logits which allows a select few tokens to be more aligned with higher resulting scores. This phenomena can be seen in \cref{fig:attention} where a small subset keys and queries contribute to the majority of the attention score. 




% In order to determine the importance of individual keys using the data contained in the attention matrix when multiple queries are used in the computation, this information must be aggregated over the query dimension. Many sparse attention methods \citep{li2024snapkv, zhu2024sampleattention, zhang2024h2o} advocate taking the mean along the query dimension. However, \cref{fig:attention} shows that in some cases, keys may only attend to a small number of queries in question but may do so quite strongly. In this case, using the mean along the query dimension can decrease the scores for such keys. This suggests that we should use the max to aggregate scores along the query dimension and because of this we only need to consider those queries that attend to most keys strongly over the sequence length. Our empirical results show that using the max to aggregate significantly outperforms mean aggregation especially when using chunked prefill. These can be seen in \cref{table:ruler_ablation}. 



% \cite{park2025keydiff} demonstrated theoretically and empirically that persistently important keys may be identified by selecting those which have lowest cosine similarity with the average key. The same pattern holds for queries, in which queries with significant attention scores across the sequence length as in \cref{fig:attention} tend to be distant in terms of cosine similarity to the average query.

% We show this choice of query subselection is optimal due to the following theorem.

% \begin{theorem}\label{theorem:keydiff-key-query}
% Consider tokens a fixed query and key ${q_0}$, $k$ and let the average of the query tokens be denoted $\bar{q}$. Suppose $\textrm{CosSim}({k}, q_0) = \beta_q > 0$ and $\textrm{CosSim}(\bar{q}, k) = \alpha_q < 0$. Then 
% \begin{equation}
% \textrm{CosSim}(\bar{q}, {q^*}) \leq 1 + \alpha_q \beta_q - 0.5\alpha_q^2 -0.5\beta_q^2.
% \label{eq:key-query-eq}
% \end{equation}
% \end{theorem}

% Proof of this result follows directly from Theorem $1$ in \cite{park2025keydiff}. 

% They also show that keys and queries tend to angularly cluster around their mean and that key means and query means tend to point in opposite directions. This means that if a query $q$ attends strongly to $k$, $\beta_q$ above will be large, $\alpha_q$ will be small and the metric we use to select the queries, $-\textrm{CosSim}(\bar{q}, {q^*})$ will be large. Hence the method we use to subselect queries should retain most of the information contained in the attention computation.








% This requires accelerating both the prefill phase \cref{sec:method_algorithm} and the \cref{sec:method_generation}.
\subsection{\ourmethod{}}
\label{sec:method_algorithm} Putting the above elements together,
\cref{alg:ourmethod} presents \ourmethod{} for fast prefill and generation. It first subselects queries based on cosine dis-similarity to the average query, aggregates the resulting queries in key-value groups, computes the cosine similarity with keys, and takes the maximum across the query dimension. 
% Our algorithm for fast prefill and generation is presented in \cref{alg:ourmethod} in which we first subselect queries based on cosine dis-similarity to the average query, aggregate the resulting queries in key-value groups, compute the cosine similarity with keys, and take the maximum across the query dimension. 
These operations can be made more or less efficient, trading off some performance loss with a decrease in latency. It should be noted that the pre-aggregation of queries makes this method viable for increasing TPS during generation as well. If $B_{CP}$ is the chunk size each step of chunked prefill using \ourmethod{} takes  $\frac{B_{CP} n_{Q}}{M_Q n_{KV}}$ less computation and memory transfer than full attention. \emph{Note that \ourmethod{} and the other selective attention methods we test are only applied on keys from the KV cache, not incoming keys from the current processing step.}

% \begin{algorithm}
% \caption{\ourmethod{}}\label{alg:ourmethod}
% \begin{algorithmic}
% \Require keys $K$, queries $Q$, values $V$, selective budget $B$, max selected queries $N_Q$, number of KV heads $n_{\mathrm{KV}}$, number of attention heads $n_{\mathrm{Q}}$
% \State \Comment{$K$, $V$ have shape $(b, n_{\mathrm{KV}}, N, d)$, $Q$ has shape $(b, n_{\mathrm{Q}}, N, d)$}
% \If{$|Q| > N_Q$}
%     \State $M_Q = \texttt{mean}(Q, \texttt{dim=2})$
%     \State $S_Q = \mathrm{CosSim}(Q, M_Q)$
%     \State $Q^\star = \texttt{gather}(\mathrm{topk}(-S_Q, N_Q), Q)$
% \Else
%     \State $Q^\star = Q$
% \EndIf

% % Faster Cosine Sim using pre-aggregation
% \State $Q = Q/\texttt{norm}(Q, \texttt{dim=-1})$
% \State $K = K/\texttt{norm}(K, \texttt{dim=-1})$
% %\State $K = normalize(K, dim = -1)$
% \State $\bar{Q} = \texttt{mean}(Q^\star.\texttt{reshape}(b, n_{\mathrm{KV}},\frac{n_{\mathrm{Q}}}{n_{\mathrm{KV}}},  N_Q, d), 
% \texttt{dim=2})$ \Comment{$(b, n_{\mathrm{KV}}, N_Q, d)$}
% \State $S = \bar{Q}K^T$ \Comment{$(b, n_{\mathrm{KV}}, N_Q, N)$} %$$S = \mathrm{CosSim}(\bar{Q}, K)$ \

% \State $\hat{S} = \texttt{max}(S, \texttt{dim=2})$ 
% \State $\hat{S}, I = \texttt{topk}(\hat{S}, B)$
% \State $K^\star = \texttt{gather}(K, I)$
% \State $V^\star = \texttt{gather}(V, I)$
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[t]
\caption{\ourmethod{}}
\label{alg:ourmethod}
\begin{algorithmic}[1]   % [1] = line numbers
\Require keys $K$, queries $Q$, values $V$, selective attention budget $B_{\text{SA}}$, 
         max queries $N_Q$, number of KV heads $n_{\mathrm{KV}}$, 
         number of attention heads $n_{\mathrm{Q}}$

\Comment{Query Sub-selection}
\If{$|Q| > N_Q$}
  \State $M_Q \gets \texttt{mean}(Q, \texttt{dim=2})$
  \State $S_Q \gets \mathrm{CosSim}(Q, M_Q)$
  \State $Q \gets \texttt{gather}(\mathrm{topk}(-S_Q, N_Q), Q)$
\Else
  \State $Q \gets Q$
\EndIf

\Comment{Efficient Cosine Similarity via Pre-aggregation}
\State $Q \gets Q / \texttt{norm}(Q, \texttt{dim=-1})$
\State $K \gets K / \texttt{norm}(K, \texttt{dim=-1})$

\State $\bar{Q} \gets \texttt{mean}\!\left(Q.\texttt{reshape}(b, n_{\mathrm{KV}}, \tfrac{n_{\mathrm{Q}}}{n_{\mathrm{KV}}}, N_Q, d), \texttt{dim=2}\right)$
\State $S \gets \bar{Q} K^\top$ \Comment{$(b, n_{\mathrm{KV}}, N_Q, N)$}
\State $\hat{S} \gets \max(S, \texttt{dim=2})$ \Comment{$(b, n_{\mathrm{KV}}, N)$}
\State $\hat{S}, I \gets \texttt{topk}(\hat{S}, B_{\text{SA}})$
\State $K^\star \gets \texttt{gather}(K, I)$
\State $V^\star \gets \texttt{gather}(V, I)$

\end{algorithmic}
\end{algorithm}


% \subsection{Generation}
% \label{sec:method_generation}
% \begin{algorithm}
% \caption{\ourmethod{} Generation}\label{alg:generation}
% \begin{algorithmic}
% \Require keys $K$, queries $Q$, values $V$, selective budget $B$, number of channels $C$, selected keys from the previous layer $I_K$
% \Comment{$I_K$ is optionally \texttt{None}}
% \If{$I_K$ is \texttt{None}}
%     \State $T = \texttt{mean}(|K|, \texttt{dim=2}) + \texttt{mean}(|Q|, \texttt{dim=2})$
%     \State $I = \texttt{topk}(T, \texttt{dim=-1})$
%     \State $\bar{K} = \texttt{gather}(K, I)$
%     \State $\bar{Q} = \texttt{gather}(Q, I)$
%     \State $S = -\mathrm{CosSim}(\bar{K}, \bar{Q})$
%     \State $I = \texttt{topk}(S, B)$
% \Else
%     \State $I = I_K$
% \EndIf
% \State $K^\star = \texttt{gather}(K, I)$
% \State $V^\star = \texttt{gather}(V, I)$

% \State \Return $K^\star$, $V^\star$
% \end{algorithmic}
% \end{algorithm}
% \subsection{Theoretical Justification?}






==> tables/ablation_cossim.tex <==
\begin{wraptable}{r}{0.5\linewidth}
% \vspace{-2mm}
\centering
\caption{Scoring Ablation}
\label{table:ruler_ablation_cossim}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccc}
\toprule

\multirow{2.5}{*}{Scoring Method} & \multicolumn{4}{c}{Ruler Test Length} \\
\cmidrule(lr){2-5} 
&
{4096} & {8192} & 
{16384} & {32768}
\\

\midrule
 Attention Logits & 83.76 & 68.22 & 57.97& 46.24\\
 Cosine Similarity & \bf{88.56} & \bf{73.78} & \bf{65.57} & \bf{52.48}\\
\hline
\end{tabular}
}
% \vspace{-2mm}
\end{wraptable}

==> tables/ablation_mean.tex <==
\begin{wraptable}{l}{0.45\linewidth}
% \vspace{-2mm}
\centering
\caption{Aggregation Ablation}
\label{table:ruler_ablation}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccc}
\toprule

\multirow{2.5}{*}{Aggregation} & \multicolumn{4}{c}{Ruler Test Length} \\
\cmidrule(lr){2-5} 
&
{4096} & {8192} & 
{16384} & {32768}
\\

\midrule
 Mean & 84.28 & 69.14 & 58.81& 45.53\\
 Max & \bf{88.56} & \bf{73.78} & \bf{65.57} & \bf{52.48}\\
\hline
\end{tabular}
}
% \vspace{-2mm}
\end{wraptable}

==> tables/longbench_compare.tex <==






\begin{table*}[!t]
\caption{\textbf{LongBench results (Higher is better)}. Raw scores reported for base models and relative errors (percent of performance compared to baseline) presented for \ourmethod{}.}

\label{table:longbench_compare}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccccccccccccc}
\toprule


&
\multicolumn{3}{c}{\bf{\ourmethod{}}} &
\multicolumn{3}{c}{\bf{Sample Attention}} &
\multicolumn{3}{c}{\bf{LessIsMore}} &
\multicolumn{3}{c}{\bf{SparQ}} &
\multicolumn{3}{c}{\bf{Loki}} &

\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}
\cmidrule(lr){11-13}
\cmidrule(lr){14-16}
\bf{Selective Budget} &
{512} & {1024} & {2048} & {512} & {1024} & {2048} & {512} & {1024} & {2048} & {512} & {1024} & {2048}& {512} & {1024} & {2048}\\
\midrule
\midrule
  {\bf{Llama3.2-3B-Instruct}} & \bf{0.945} & \bf{0.972} & \bf{0.986} & 0.738 & 0.80 & 0.901 & 0.703 & 0.788 & 0.85 & 0.721 & 0.802 & 0.842 & 0.686 & 0.757 & 0.842 \\ 
% \midrule 
% \bf{Qwen2.5-3B-Instruct}
%  \\

% \midrule
\midrule
\bf{Qwen2.5-3B-Instruct} & \bf{0.869} & \bf{0.945} & \bf{0.977} & 0.660 & 0.756 & 0.828 & 0.461 & 0.556 & 0.659 & 0.636 & 0.726 & 0.808 & 0.589 & 0.671 & 0.787 \\
\midrule 

% \bf{Qwen3-4B}
%  \\

% \midrule
% \midrule
 \textcolor{red}{\bf{Qwen3-4B} &\bf{0.998} & \bf{1.03} & \bf{1.028} & 0.856 & 0.929 & 0.966 & 0.765 & 0.842 & 0.918 & 0.725 & 0.805 & 0.922 & 0.384 & 0.801 & 0.622 }\\
\midrule
 \bf{Smollm3} &\bf{0.998} & \bf{1.03} & \bf{1.028} & 0.856 & 0.929 & 0.966 & 0.765 & 0.842 & 0.918 & 0.725 & 0.805 & 0.922 & 0.384 & 0.801 & 0.622\\


\bottomrule
\end{tabular}
}
\vspace{-5mm}
\end{center}
\end{table*}


==> tables/longbench_ggattn.tex <==
\begin{table*}[!t]
\caption{\textbf{LongBench results (Higher is better)}. Raw scores reported for base models and relative errors (percent of performance compared to baseline) presented for \ourmethod{}.}


\label{table:longbench_ggattn}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{c | ccc ccc ccc ccc ccc ccc}
\toprule


&
\multicolumn{3}{c}{\bf{Llama3.1-8B-Instruct}} &
\multicolumn{3}{c}{\bf{Llama3.2-3B-Instruct}} &
\multicolumn{3}{c}{\bf{Qwen2.5-3B-Instruct}} &
\multicolumn{3}{c}{\bf{Qwen3-4B}} &
\multicolumn{3}{c}{\bf{Qwen3-1.7B}} &
\multicolumn{3}{c}{\bf{Smollm3}} &

\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}
\cmidrule(lr){11-13}
\cmidrule(lr){14-16}
\cmidrule(lr){17-19}
\bf{Selective Budget} &
{512} & {1024} & {2048}  &  {512} & {1024} & {2048} &  {512} & {1024} & {2048}&  {512} & {1024} & {2048}&  {512} & {1024} & {2048}&  {512} & {1024} & {2048}\\% & {2048} & {512} & {1024} & {2048} & {512} & {1024} & {2048}& {512} & {1024} & {2048}\\
\midrule
\midrule
  \bf{Normalized Score} 
  & 0.962 & 0.977 & 0.992 & 
  0.945 & 0.972  & 0.986 & 
  0.869 & 0.945  & 0.977& 
  0.966 & 0.992  & 0.995& 
  0.953 & 0.984  & 0.986& 
  0.998 & 1.03  & 1.028\\ %& 0.901 & 0.703 & 0.788 & 0.85 & 0.721 & 0.802 & 0.842 & 0.686 & 0.757 & 0.842 \\ 
% \midrule 
% \bf{Qwen2.5-3B-Instruct}
%  \\

% \midrule
% \cmidrule(lr){2-7}
%  & 0.869 & 0.945 & 0.977 & 0.660 & 0.756  & 0.869& 0.660 & 0.756  & 0.869& 0.660 & 0.756  & 0.869& 0.660 & 0.756  & 0.869& 0.660 & 0.756  & 0.869 \\%& 0.828 & 0.461 & 0.556 & 0.659 & 0.636 & 0.726 & 0.808 & 0.589 & 0.671 & 0.787 \\
% \cmidrule(lr){2-7}

% \bf{Qwen3-4B}
%  \\

% \mid


\bottomrule
\end{tabular}
}
\vspace{-5mm}
\end{center}
\end{table*}


==> tables/ruler_compare.tex <==
% \begin{table*}[!t]
% \caption{\textbf{Ruler Results} across different models and selective attention methods. All experiments use chunked prefill with $B=128$ and selective budget $1024$.}
% \label{table:ruler_compare}
% \begin{center}
% \resizebox{.55\textwidth}{!}{
% \begin{tabular}{c | c | ccccc}
% \toprule

% {Model} & 
% {Method} &
% {4096} & {8192} & 
% {16384} & {32768}
% \\


% \midrule
% \multirow{7}{*}{Llama-3.2-3B}
% & SnapKV & 29.15 & 13.70 & NA & NA\\
% & KeyDiff & 53.34 & 31.102 & NA& NA\\
% & SampleAttention & 78.25 & 61.14 & 48.31& 31.73\\
% & TidalDecode & 75.15 & 49.23 & 30.44& 19.16\\
% & Loki & 74.84 & 56.50 & 25.76& 8.05\\
% & SparQ & 75.15 & 49.23 & 30.44& 19.16\\
% & SPARK & \bf{88.56} & \bf{73.78} & \bf{65.57}& \bf{52.48}\\
% \midrule
% \multirow{7}{*}{Llama-3.1-3B}
%   & SnapKV & 37.23 & 13.22 & 7.61 & 3.17\\
% & KeyDiff & 67.54 & 40.91 & 22.21 & 16.73\\
% & SampleAttention & 85.12 & 73.87 & 60.85& 48.02\\
% & TidalDecode & 83.93 & 60.47 & 43.56 & 26.35\\
% & Loki & 81.03 & 67.55 &61.36& 38.80\\
% & SparQ & 84.62 & 72.53 & 62.52& 48.53\\
% & SPARK & \bf{89.97} & NA & NA& NA\\
% \midrule






% \multirow{7}{*}{Qwen-2.5-3B}
%   & SnapKV & 19.25 & 12.40 & 9.88 & 8.13\\
% & KeyDiff & 34.09 & 20.68 & 15.79 & 10.32\\
% & SampleAttention & 77.17 & 60.88 & 56.64& 36.17\\
% & TidalDecode & 36.66 & 20.21 & 12.84 & 10.12\\
% & Loki & 74.40 & 60.09 & 48.96 & 34.12\\
% & SparQ & 78.07 & 59.87 & 54.71 & 36.74\\
% & SPARK & \bf{84.05} & \bf{68.72} & \bf{62.60}& \bf{48.34} \\

% \midrule

% \multirow{7}{*}{Qwen-3-4B}
%   & SnapKV & 27.29 & 17.15 & 10.94 & 10.07\\
% & KeyDiff & 37.29 & 27.15 & 20.94 & 12.07\\
% & SampleAttention & 87.84 & 72.46 & 59.57& 40.72\\
% & TidalDecode & 65.55 & 42.75 & 24.39& 14.87\\
% & Loki & 82.83 & 65.19 & 52.29& 39.31\\
% & SparQ & 87.93 & 68.97 & 56.02& 35.20\\
% & SPARK & \bf{91.78} & \bf{81.72} & \bf{70.18}& \bf{63.12}\\


% \midrule

% \multirow{7}{*}{Smollm3}
%   & SnapKV & NA & NA & NA & NA\\
% & KeyDiff & NA & NA & NA& NA\\
% & SampleAttention & 85.72 & 66.44 & 59.10& 45.98\\
% & TidalDecode & 79.67 & 50.17 & 35.12& 24.21\\
% & Loki & 84.52 & 64.20 & 50.10& 22.66\\
% & SparQ & 82.45 & 57.62 & 32.18& 18.69\\
% & SPARK & \bf{89.56} & \bf{76.29} & \bf{69.16}& \bf{57.79}\\
% \bottomrule

% \end{tabular}
% }



% \end{center}
% \end{table*}


\noindent
\begin{minipage}[t]{0.49\textwidth}

\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c | c | cccc}
\toprule
\multirow{2.5}{*}{Model} & 
\multirow{2.5}{*}{Method} & \multicolumn{4}{c}{Ruler Test Length} \\
\cmidrule(lr){3-6}

 & 
 &
{4096} & {8192} & 
{16384} & {32768}
\\


\midrule
\multirow{7}{*}{Llama-3.2-3B}
& SnapKV & 29.15 & 13.70 & 12.44 & 6.21\\
& KeyDiff & 53.34 & 31.10 & 24.29& 14.87\\
& SampleAttention & 78.25 & 61.14 & 48.31& 31.73\\
& TidalDecode & 75.15 & 49.23 & 30.44& 19.16\\
& Loki & 74.84 & 56.50 & 25.76& 8.05\\
& SparQ & 75.15 & 49.23 & 30.44& 19.16\\
& \ourmethod{} & \bf{88.56} & \bf{73.78} & \bf{65.57}& \bf{52.48}\\
\midrule
\multirow{7}{*}{Llama-3.1-3B}
  & SnapKV & 37.23 & 13.22 & 7.61 & 3.17\\
& KeyDiff & 67.54 & 40.91 & 22.21 & 16.73\\
& SampleAttention & 85.12 & 73.87 & 60.85& 48.02\\
& TidalDecode & 83.93 & 60.47 & 43.56 & 26.35\\
& Loki & 81.03 & 67.55 &61.36& 38.80\\
& SparQ & 84.62 & 72.53 & 62.52& 48.53\\
& \ourmethod{} & \bf{89.24} & \bf{89.51} & \bf{83.25} & \bf{70.04} \\
\midrule


\multirow{7}{*}{Qwen-2.5-3B}
  & SnapKV & 19.25 & 12.40 & 9.88 & 8.13\\
& KeyDiff & 34.09 & 20.68 & 15.79 & 10.32\\
& SampleAttention & 77.17 & 60.88 & 56.64& 36.17\\
& TidalDecode & 36.66 & 20.21 & 12.84 & 10.12\\
& Loki & 74.40 & 60.09 & 48.96 & 34.12\\
& SparQ & 78.07 & 59.87 & 54.71 & 36.74\\
& \ourmethod{} & \bf{84.05} & \bf{68.72} & \bf{62.60}& \bf{48.34} \\

\midrule

\multirow{7}{*}{Qwen-3-4B}
  & SnapKV & 27.29 & 17.15 & 10.94 & 10.07\\
& KeyDiff & 37.29 & 27.15 & 20.94 & 12.07\\
& SampleAttention & 87.84 & 72.46 & 59.57& 40.72\\
& TidalDecode & 65.55 & 42.75 & 24.39& 14.87\\
& Loki & 82.83 & 65.19 & 52.29& 39.31\\
& SparQ & 87.93 & 68.97 & 56.02& 35.20\\
& \ourmethod{} & \bf{91.78} & \bf{81.72} & \bf{70.18}& \bf{63.12}\\


\midrule

\multirow{7}{*}{Smollm3}
  & SnapKV & 43.72 & 35.98 & 24.21 & 12.23\\
& KeyDiff & 62.85 & 51.60 & 41.64& 30.37\\
& SampleAttention & 85.72 & 66.44 & 59.10& 45.98\\
& TidalDecode & 79.67 & 50.17 & 35.12& 24.21\\
& Loki & 84.52 & 64.20 & 50.10& 22.66\\
& SparQ & 82.45 & 57.62 & 32.18& 18.69\\
& \ourmethod{} & \bf{89.56} & \bf{76.29} & \bf{69.16}& \bf{57.79}\\
\bottomrule


\end{tabular}
}

\captionof{table}{\textbf{Ruler Results} across different models and selective attention methods. All experiments use selective budget $1024$. Results in {\bf{bold}} represent the best across model and selective attention method.}
\label{table:ruler_compare}
\end{minipage}
\hfill
\begin{minipage}[t]{0.49\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c | c | cccc}
\toprule
\multirow{2.5}{*}{Model} & 
\multirow{2.5}{*}{Budget} & \multicolumn{4}{c}{Ruler Test Length} \\
\cmidrule(lr){3-6}

 & 
 &
{4096} & {8192} & 
{16384} & {32768}
\\


\midrule
\multirow{4}{*}{Llama-3.2-3B}
& Full & 87.50 & 81.33 & 76.98 & 74.31\\
& 4096 & 87.51 & 80.60 & 75.69 & 69.95\\
& 2048 & 87.33 & 80.20 & 73.79 & 63.67\\
& 1024 & 86.71 & 80.19 & 70.90 & 57.01\\
\midrule

\multirow{4}{*}{Llama-3.1-3B}
& Full & 89.45 & 90.24 & 90.53 & 86.65\\
& 4096 & 89.45 & 89.03 & 87.46 & 81.33\\
& 2048 & 89.20 & 88.82 & 86.21 & 78.86 \\
& 1024 & 89.24 & 89.51 & 83.25 & 70.04 \\
\midrule



\multirow{4}{*}{Qwen-2.5-3B}
& Full & 89.57 & 81.99 & 76.09 & 71.69\\
& 4096 & 89.53 & 81.53 & 74.83 & 68.43\\
& 2048 & 89.56 & 79.41 & 71.13 & 63.82\\
& 1024 & 87.85 & 68.72& 62.60& 48.34\\
\midrule



\multirow{4}{*}{Qwen-3-4B}
& Full & 93.32 & 91.68 & 91.18 & 88.54\\
& 4096 & 93.32 & 91.83 & 91.06 & 87.68\\
& 2048 & 93.13 & 91.80 & 88.87 & 85.23\\
& 1024 & 91.78 & 81.72 & 70.18 & 63.12\\
\midrule



\multirow{4}{*}{Smollm3}
& Full & 91.21 & 83.46 & 80.11 & 75.18\\
& 4096 & 91.21 & 83.70 & 79.66 & 71.83\\
& 2048 & 90.96 & 83.06 & 78.26 & 67.65\\
& 1024 & 89.56 & 76.29 & 69.16 & 57.79\\
\bottomrule


\end{tabular}
}
\captionof{table}{Ruler Results \ourmethod{} comparing full cache performance with different selective budgets.}
\label{table:ruler_ggattn}
\end{minipage}

==> tables/ruler_compare_unrolled.tex <==
% \begin{table}[t]
\vspace{-7mm}
\hspace{-9mm}
\begin{wraptable}{l}{.95\linewidth}
\centering
\caption{{\textbf{Ruler results} \newline \footnotesize{Comparisons of different models and different cache policies on the RULER benchmark across different test lengths using selective budget $1024$. Highest scores in {\bf{bold}.}}}}
\label{tab:ruler_transposed_all}
\footnotesize
% \renewcommand{\arraystretch}{0.5}
\resizebox{.4\textwidth}{!}{
\begin{tabular}{l c c c c c c c}
\toprule

& \multicolumn{2}{c}{\textit{Token Eviction}} & \multicolumn{5}{c}{\textit{Sparse Attention}} \\

\cmidrule(lr){2-3} \cmidrule(lr){4-8}

Length &
%\textit{Dense} &
SnapKV &
KeyDiff &
SampleAttn &
LessIsMore &
Loki &
SparQ &
\ourmethod{} \\
\midrule


\multicolumn{8}{c}{\textit{Llama-3.2-3B-Instruct}} \\
\midrule
4,096   & 29.15 & 53.34 & 78.25 & 75.15 & 74.84 & 75.15 & {\bfseries 86.71} \\
8,192   & 13.70 & 31.10 & 61.14 & 49.23 & 56.50 & 49.23 & {\bfseries 80.19} \\
16,384  & 12.44 & 24.29 & 48.31 & 30.44 & 25.76 & 30.44 & {\bfseries 70.90} \\
32,768 &  6.21 & 14.87 & 31.73 & 19.16 &  8.05 & 19.16 & {\bfseries 57.01} \\
\midrule


% \multicolumn{8}{c}{\textit{Llama-3.1-8B-Instruct}} \\
% \midrule
% 4,096   & 37.23 & 67.54 & 85.12 & 83.93 & 81.03 & 84.62 & {\bfseries 89.97} \\
% 8,192  & 13.22 & 40.91 & 73.87 & 60.47 & 67.55 & 72.53 & {\bfseries 83.96} \\
% 16,384  &  7.61 & 22.21 & 60.85 & 43.56 & 61.36 & 62.52 & {\bfseries 77.37} \\
% 32,768  &  3.17 & 16.73 & 48.02 & 26.35 & 38.80 & 48.53 & {\bfseries 63.66} \\
% \midrule

\multicolumn{8}{c}{\textit{Qwen-2.5-3B}} \\
\midrule
4,096   & 19.25 & 34.09 & 77.17 & 36.66 & 74.40 & 78.07 & {\bfseries 87.85} \\
8,192   & 12.40 & 20.68 & 60.88 & 20.21 & 60.09 & 59.87 & {\bfseries 74.27} \\
16,384 &  9.88 & 15.79 & 56.64 & 12.84 & 48.96 & 54.71 & {\bfseries 66.82} \\
32,768 &  8.13 & 10.32 & 36.17 & 10.12 & 34.12 & 36.74 & {\bfseries 59.37} \\
\midrule


\multicolumn{8}{c}{\textit{Qwen-3-4B}} \\
\midrule
4,096  & 27.29 & 37.29 & 87.84 & 65.55 & 82.83 & 87.93 & {\bfseries 93.73} \\
8,192  & 17.15 & 27.15 & 72.46 & 42.75 & 65.19 & 68.97 & {\bfseries 91.07} \\
16,384  & 10.94 & 20.94 & 59.57 & 24.39 & 52.29 & 56.02 & {\bfseries 88.57} \\
32,768 & 10.07 & 12.07 & 40.72 & 14.87 & 39.31 & 35.20 & {\bfseries 74.83} \\
\midrule

\multicolumn{8}{c}{\textit{Smollm3}} \\
\midrule
4,096  & 43.72 & 62.85 & 85.72 & 79.67 & 84.52 & 82.45 & {\bfseries 89.97} \\
8,192  & 35.98 & 51.60 & 66.44 & 50.17 & 64.20 & 57.62 & {\bfseries 79.94} \\
16,384  & 24.21 & 41.64 & 59.10 & 35.12 & 50.10 & 32.18 & {\bfseries 72.69} \\
32,768  & 12.23 & 30.37 & 45.98 & 24.21 & 22.66 & 18.69 & {\bfseries 61.37} \\


\bottomrule
\end{tabular}
}
\end{wraptable}
% \end{table}

